Capturing Power System Dynamics by Physics-Informed Neural Networks and Optimization

This paper proposes a tractable framework to determine key characteristics of non-linear dynamic systems by converting physics-informed neural networks to a mixed integer linear program. Our focus is on power system applications. Traditional methods in power systems require the use of a large number of simulations and other heuristics to determine parameters such as the critical clearing time, i.e. the maximum allowable time within which a disturbance must be cleared before the system moves to instability. The work proposed in this paper uses physics-informed neural networks to capture the power system dynamic behavior and, through an exact transformation, converts them to a tractable optimization problem which can be used to determine critical system indices. By converting neural networks to mixed integer linear programs, our framework also allows to adjust the conservativeness of the neural network output with respect to the existing stability boundaries. We demonstrate the performance of our methods on the non-linear dynamics of converter-based generation in response to voltage disturbances.

==> 25_discussion.tex <==
The presented results showcase the flexibility of the proposed framework to choose the objective function and constraints such that we can extract meaningful information about the system. While running a large number of time-domain simulations could yield similar insights, the associated computational burden eliminates this option as soon as we move into higher dimensions in the input domain. To lower the computation burden, the search space of the input domain could be screened using PINNs which can accelerate the function evaluation process by several orders of magnitude. However, such a procedure still requires targeted search algorithms. The presented framework avoids this by rigorously analyzing the search space using optimization.

A central question of concern is how to verify the approximation of the PINN or guarantee a certain behaviour. A way forward could be guarantees along the lines of \cite{venzke2020learning}, \cite{Venzke2020verification} to certify that the PINN behaves within defined bounds. While this is not to be confused with guaranteeing that the PINN is exact with respect to the ground truth, such certificates supersede simple heuristic analyses. The presented framework is easily adjustable towards answering these questions. A more straightforward path to judge the quality of the approximations of the PINN is to use knowledge about the dynamical system to perform multiple analysis from different angles as in \cref{sec:results} that should lead to matching conclusions.  

For higher dimensional input domains, e.g. including system parameters, the framework could allow to quickly identify regions of interest that can be screened more thoroughly by simply evaluating PINNs at selected points. The benefits of the rigorous approach could become useful in multi-objective problems.
